Measurement of \gamma\ from B->Dh decays at LHCb---including the effect of D0-D0bar mixing

I present a measurement of the CKM angle gamma from a combination of three LHCb measurements using the tree decays B -> DK and B -> Dpi. These measurements are based on a dataset corresponding to 1.0fb-1, collected in 2011. In contrast to what was presented at FPCP, these proceedings fully include the effect of D0--D0b mixing on the combination. I also report on the inclusion of new, preliminary results on the Dalitz analysis of B->DK, D->KShh, using a dataset corresponding to 3fb-1, collected in 2011--2012.

==> Makefile <==

# keep secondary files
.SECONDARY:
	

# name of the main latex file (do not include .tex)
MAIN = mkarbach

# prescription how to make output (your favorite commands to process latex)
# We need to include %.tex in the prerequisites to enable creation of main_linenum.tex.
%.pdf: %.tex $(filter-out %.tex, $(wildcard *.tex)) $(wildcard *.bib)
	pdflatex $* && \
	bibtex	 $* && \
	pdflatex $* && \
	pdflatex $*
	@echo
	@egrep -i --color "(Reference|Citation|multiply).*defined" $(@:%.pdf=%.log); true


# add line numbers
%_linenum.tex: $(filter-out $(MAIN)_linenum.tex, $(wildcard *.tex)) $(wildcard *.bib)
	./add_linenum $*.tex


# remove comments
%_nocomments.tex: %.tex $(filter-out %.tex, $(wildcard *.tex)) $(wildcard *.bib)
	perl -e 'while(<>){next if m/^\s*%/; s/([^\\])%.*$ /$$1/g; print;}' < $< > $@


default: $(MAIN)_linenum.pdf
	

all: $(MAIN)_linenum.pdf $(MAIN).pdf
	

.PHONY: clean rmout new fresh

# remove temporary files (good idea to say "make clean" before putting things back into repository)
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.toc *.out $(MAIN)_linenum.tex $(MAIN)_nocomments.tex lineno_babar.sty

# remove output file
rmout: 
	rm -f $(MAIN).pdf $(MAIN)_linenum.pdf

# some handy aliases
new: fresh default
	
fresh: clean rmout
	

